Beyond 5G RIS mmWave Systems: Where Communication and Localization Meet

Upcoming beyond fifth generation (5G) communications systems aim at further enhancing key performance indicators and fully supporting brand new use cases by embracing emerging techniques, e.g., reconfigurable intelligent surface (RIS), integrated communication, localization, and sensing, and mmWave/THz communications. The wireless intelligence empowered by state-of-the-art artificial intelligence techniques has been widely considered at the transceivers, and now the paradigm is deemed to be shifted to the smart control of radio propagation environment by virtue of RISs. In this article, we argue that to harness the full potential of RISs, localization and communication must be tightly coupled. This is in sharp contrast to 5G and earlier generations, where localization was a minor additional service. To support this, we first introduce the fundamentals of RIS mmWave channel modeling, followed by RIS channel state information acquisition and link establishment. Then, we deal with the connection between localization and communications, from a separate and joint perspective.

==> Figs/Fig5.tex <==
\begin{tikzpicture}[every text node part/.style={align=center}]
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
\node [rotate = 90] at (-2.2cm,2cm){\footnotesize $y (\mathrm{m})$};
\node [rotate = 0] at (.8cm,4.1cm){\footnotesize a) random, PEB $ (\mathrm{m})$};
\node [rotate = 0] at (6.3cm,4.1cm){\footnotesize b) random, SE $ (\mathrm{bits/s/Hz})$};
\node [rotate = 0] at (11.5cm,4.1cm){\footnotesize c) directional, SE $ (\mathrm{bits/s/Hz})$};

%%---------first image------------
\begin{axis}[
at={(-1.4cm,0cm)},
axis on top,% ----
width=8*.62*.8cm,
height=6*.8*.8cm,
xlabel={\footnotesize $x (\mathrm{m})$},
scale only axis,
xmin=-10,
xmax=10,
ymin=0,
ymax=10,
enlargelimits=false, 
axis on top, 
]
\addplot[thick,blue] graphics[xmin=-10,ymin=0,xmax=10,ymax=10] {Figs/F5_random_PEB.eps};
\end{axis}
\begin{axis}[at={(2.7cm,0cm)},axis on top,% ----
		width=.5*.6cm,
		height=6*.8*.8cm,
		scale only axis,
		xmin=0,
		xmax=1,
		ymin=1e-4,
		ymax=1,
		ymode = log,
		xtick=\empty,
		%ytick={0,-1,-2,-3,-4},
        %yticklabels={$10^0$,$10^{-1}$,$10^{-2}$,$10^{-3}$,$10^{-4}$},
		enlargelimits=false, 
		axis on top, 
        ytick pos=right,
]
\addplot[thick,blue] graphics[xmin=0,ymin=1e-4,xmax=1,ymax=1] {F5_random_PEB_clb.png};
\end{axis}
%--------------------------------------------

%%---------second image------------
\begin{axis}[
at={(4.1cm,0cm)},
axis on top,% ----
width=8*.62*.8cm,
height=6*.8*.8cm,
xlabel={\footnotesize $x (\mathrm{m})$},
scale only axis,
xmin=-10,
xmax=10,
ymin=0,
ymax=10,
ytick={0,2,4,6,8,10},
yticklabel=\empty,
enlargelimits=false, 
axis on top, 
]
\addplot[thick,blue] graphics[xmin=-10,ymin=0,xmax=10,ymax=10] {Figs/F5_random_Rate.eps};
\end{axis}
\begin{axis}[at={(8.2cm,0cm)},axis on top,% ----
		width=.5*.6cm,
		height=6*.8*.8cm,
		scale only axis,
		xmin=0,
		xmax=1,
		ymin=0.0361,
		ymax=1,
		%ymode=log,
		xtick=\empty,
		%ytick={-10,-5,0,5,10},
		enlargelimits=false, 
		axis on top, 
ytick pos=right,
]
\addplot[thick,blue] graphics[xmin=0,ymin=0.0361,xmax=1,ymax=1] {Figs/F5_random_rate_clb.png};
\end{axis}
%------------------------------------------

%%---------third image------------
\begin{axis}[
at={(9.4cm,0cm)},
axis on top,% ----
width=8*.62*.8cm,
height=6*.8*.8cm,
xlabel={\footnotesize $x (\mathrm{m})$},
ytick={0,2,4,6,8,10},
yticklabel=\empty,
scale only axis,
xmin=-10,
xmax=10,
ymin=0,
ymax=10,
enlargelimits=false, 
axis on top, 
]
\addplot[thick,blue] graphics[xmin=-10,ymin=0,xmax=10,ymax=10] {Figs/F5_directional_Rate.eps};
\end{axis}
\begin{axis}[at={(13.5cm,0cm)},axis on top,% ----
		width=.5*.6cm,
		height=6*.8*.8cm,
		scale only axis,
		xmin=0,
		xmax=1,
		ymin=1.2841,
		ymax=10,
		xtick=\empty,
		%ytick={-10,-5,0,5,10},
		enlargelimits=false, 
		axis on top, 
ytick pos=right,
]
\addplot[thick,blue] graphics[xmin=0,ymin=1.2841,xmax=1,ymax=10] {Figs/F5_directional_rate_clb.png};
\end{axis}
%--------------------------------------------
\end{tikzpicture}

